SCOPE: Structural Continuity Preservation for Medical Image Segmentation

Although the preservation of shape continuity and physiological anatomy is a natural assumption in the segmentation of medical images, it is often neglected by deep learning methods that mostly aim for the statistical modeling of input data as pixels rather than interconnected structures. In biological structures, however, organs are not separate entities; for example, in reality, a severed vessel is an indication of an underlying problem, but traditional segmentation models are not designed to strictly enforce the continuity of anatomy, potentially leading to inaccurate medical diagnoses. To address this issue, we propose a graph-based approach that enforces the continuity and connectivity of anatomical topology in medical images. Our method encodes the continuity of shapes as a graph constraint, ensuring that the network's predictions maintain this continuity. We evaluate our method on two public benchmarks on retinal vessel segmentation, showing significant improvements in connectivity metrics compared to traditional methods while getting better or on-par performance on segmentation metrics.

==> SCOPE_ arXiv/chapters/0_abstract.tex <==
\begin{abstract}
Although the preservation of shape continuity and physiological anatomy is a natural assumption in the segmentation of medical images, it is often neglected by deep learning methods that mostly aim for the statistical modeling of input data as pixels rather than interconnected structures. In biological structures, however, organs are not separate entities; for example, in reality, a severed vessel is an indication of an underlying problem, but traditional segmentation models are not designed to strictly enforce the continuity of anatomy, potentially leading to inaccurate medical diagnoses. To address this issue, we propose a graph-based approach that enforces the continuity and connectivity of anatomical topology in medical images. Our method encodes the continuity of shapes as a graph constraint, ensuring that the network's predictions maintain this continuity. We evaluate our method on two public benchmarks on retinal vessel segmentation, showing significant improvements in connectivity metrics compared to traditional methods while getting better or on-par performance on segmentation metrics.

%\keywords{Continuity Preservation  \and Vessel segmentation \and Graphs.}
\end{abstract}


\iffalse
The preservation of shape continuity is a critical aspect of medical imaging, yet it is often neglected by deep learning-based methods. In biological structures, organs are not separate entities, and maintaining continuity in structures such as veins is essential. However, traditional deep learning methods do not enforce this continuity, potentially leading to inaccurate medical diagnoses. To address this issue, we propose a graph-based approach that enforces continuity in medical images. Our method encodes the continuity of shapes as a graph constraint, ensuring that the network's predictions maintain this continuity. We evaluate our method on three datasets, showing significant improvements in shape continuity metrics compared to traditional methods while getting better or on-par performance on segmentation metrics.

\fi

==> SCOPE_ arXiv/chapters/1_introduction.tex <==
\section{Introduction}
Deep learning models for medical image analysis are mostly designed to prioritize the statistical modeling of shapes and textures over the morphology of the medical images. Even though the disruption of organs like vessels is often an indication of an underlying disorder, they are often ignored in favor of overall segmentation performance. The importance of modeling structural integrity becomes more prominent for the diagnosis of sensitive organs, such as the eyes, which contain dense vasculature and pose an even greater challenge. That is why such models are mostly evaluated and applied in analyzing fundus images. Although deep learning-based methods have improved the performance in retinal vessel segmentation \cite{guo2021sa,kamran2021rv,zhou2021study}, they often fail to preserve the continuity of shapes, which is crucial for accurate medical analysis. To address this, we propose a novel graph-based approach that enforces shape continuity for image segmentation.

Previous studies have attempted to incorporate topological information into retinal vessel segmentation. One such approach is to design specific loss functions that penalize the disconnectedness of segmented retinal vessels. For example, Yan et al.~\cite{yan2018joint} proposed joint segment-level and pixel-wise losses, which emphasize the thickness consistency of thin vessels. Shit et al.~\cite{shit2021cldice} developed the Centerline Dice (clDice) for tubular structures, a connectivity-aware similarity metric that improves segmentation results with more accurate connectivity information. Some studies have suggested topological objective functions to improve deep-learning models to produce results that have more similar topology as the ground truth, which help to reduce topological errors \cite{clough2020topologicalBetti,zhang2022topology}.

Other approaches incorporate architectures \cite{zhang2018road,alom2019recurrent,liu2022full} that aim to maintain the spatial information in the image. The shape conservation can be improved by either introducing residual connections \cite{zhuang2018laddernet,li2020iternet} or by using deformation-based architectures that rely on a prior mask with the same topological features as the ground truth. For example, Zhang et al.~\cite{zhang2022topology} proposed the TPSN, in which a deformation map generated from an encoder-decoder architecture transforms the template mask into the region of interest. Wyburd et al.~\cite{wyburd2021teds} also developed TEDS-Net on a continuous diffeomorphic framework.

Structural graph neural networks provide another way to model the connectivity and continuity of biological structures. Shin et al.~\cite{shin2019deep} integrated a graph attention network \cite{velivckovic2017graph} into a convolutional neural network to exploit both local properties and global vessel structures. Li et al.~\cite{9562259} extended such models to segment 3D hepatic vessels and modified the network to learn graphical connectivity from the ground truth directly. Yu et al.~\cite{yu2022vessel} maintained vessel topology by constructing edges and predicting links between different nodes generated from semantic information extracted from U-Net \cite{ronneberger2015u}; however, many medical image segmentation models aim to improve their efficiency in pixel-wise accuracy rather than modeling the connectivity and preserving continuity.
To this end, we propose a novel graph-based approach that enforces shape continuity in medical image segmentation. Our method encodes the continuity of shapes as a graph constraint, ensuring that the network's predictions maintain this continuity. Our proposed graph-based model is agnostic to prior CNN segmentation \cite{simonyan2014very}, as opposed to other graph construction approaches in previous works, such as VGN \cite{shin2019deep}. 


\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/SCOPE_pipeline.pdf}
    \caption{The visual graph is constructed using patches and 1-level edge connections in (A), node features are generated in (B), graph features are extracted in (C) and combined with initial spatial features using skip connections, and final image segmentation is produced in (D) by extending node predictions into corresponding patches.}
    \label{fig:framework}
\end{figure}

Our model directly addresses the issue of preserving shape continuity in medical image segmentation. Unlike previous approaches that rely on selecting the pixel with the highest probability in non-overlapping regions \cite{shin2019deep,velivckovic2017graph,9562259,yu2022vessel}, our method treats the patches in the image as a node for graph construction, resulting in a more efficient approach. We incorporate the DRIU \cite{maninis2016deep} architecture, utilize a graph convolution module during the learning stage, and leverage the clDice loss function \cite{shit2021cldice} to optimize our model performance. Contrary to CNN models, in which the information from the input can affect the inference, by enforcing the relation of neighboring patches of the image via message passing, we inherently bound each part of the input to the neighboring patches affecting the final inference, which our ablation studies on patch size also confirm it. Through comprehensive evaluation, we demonstrate that our approach significantly improves shape continuity metrics compared to the baselines while maintaining comparable or better performance on pixel-wise segmentation metrics. 
%Our proposed approach has the potential to improve the accuracy of medical analysis by preserving the continuity of shapes, which is critical for the accurate diagnosis and treatment of retinal diseases.

% 

==> SCOPE_ arXiv/chapters/3_methodology.tex <==
\section{Methodology}
In this section, we present our continuity preservation network. First, we introduce the overview of the proposed framework (also see \autoref{fig:framework}). Then, we elaborate on the components of our visual graph based on continuity-aware feature generators for the topology of the vessel network.


\subsection{Continuity Preservation Framework}
We design our continuity preservation framework based on graph neural networks (GNNs) \cite{scarselli2008graph} to capture the existing topology of anatomies, such as vessels in the spatial domain. The input image $x \in \mathbb{R}^{H\,\times\,W}$ is divided  into non-overlapping $n \times n$ patches. Each patch, represented as an individual graph vertex $v_i$, connects to its corresponding 1-level neighboring vertices by the edges of a fully-connected graph denoted with the adjacency matrix $A \in \mathbb{R}^{H/n \, \times \, W/n}$, where $H$ and $N$ are the image height and width respectively. The graph representation comprises $N$ vertices, with each vertex responsible for predicting its corresponding $n \times n$ sized patch. To generate initial node-level features for these vertices, inspired by DRIU \cite{maninis2016deep}, we designed a node feature generator $F_c(.)$  that receives the input image, extracts its pixel-wise features, and maps them into node-level features as vertex feature initialization. Then, graph construction module $G(.)$ fuses all sampled graph nodes with their corresponding feature vectors to complete this graph construction process, where $g_{\{A, \, f_{c}\}} = G(x, F_c(x))$. The generated features hold geometrical information about the vertices enabling them to represent general structures of  the organs like vessels; however, they do not enforce any constraints over their relations. To introduce topological information graph convolution module $F_g(.)$ extracts node-level graph features and combines them with their initial spatial features to make final class predictions for the nodes $\hat{y} \in  \mathbb{R}^{N \times 2}$ given ground-truth labels $y \in  \mathbb{R}^{N}$, where $\hat{y} = F_g(A, \, f_{c})$.


\paragraph{Graph Construction}: To construct the visual graph, we first define an image grid of non-overlapping, equally-sized, square $n \times n$ patches, where each patch serves as a vertex of the graph. This results in a vertex set $V = {v_i}^N_{i=1}$, where $N = H/n , \times , W/n$ in an input image $x \in \mathbb{R}^{H ,\times,W}$, as shown in \autoref{fig:framework}-A. Each vertex is descriptive of its corresponding patch and is initialized with feature vectors generated for each of those patches.

We introduce a direct edge construction strategy in which each vertex is connected to all 1-level neighboring vertices of its surrounding patches by undirected and unweighted edges. To capture the neighborhood in every direction, we include not only vertical and horizontal connections but also diagonal edges between the vertices. Previous works \cite{shin2019deep,yu2022vessel} have used geodesic distance to understand the geometry of retinal vessel networks, as it helps identify vertices on vessels that are closer to each other. However, since we sample the vertices everywhere to investigate the entire image region in a granular grid form, we do not use this metric. Instead, we use direct, unconstrained connections, which eliminates the necessity of geodesic vessel interpretation.

\paragraph{Node Feature Generation}: Node feature generation is a crucial step in our architecture, as it maps the pixel-wise features to the corresponding vertex-level features. We follow the approach proposed by Maninis et al. \cite{maninis2016deep}, where a VGG-16 backbone \cite{simonyan2014very} is used to extract the spatial features of a retinal fundus image $x \in \mathbb{R}^{H ,\times,W}$. We obtain a multi-level feature representation $f \in \mathbb{R}^{H ,\times, W ,\times,64}$ from the VGG backbone, capturing both local and global pixel-wise features. To generate the node-level features for our graph, we modify the DRIU architecture \cite{maninis2016deep} by replacing the $1 \times 1$ convolution with a max-pool layer of $n \times n$ window and a stride of $n$, where $n$ is the patch size. This operator downsamples the pixel-wise feature maps to a resolution of $H/n \times W/n$, generating node-level feature maps $f_{c} \in \mathbb{R}^{H/n ,\times, W/n ,\times,64}$. By applying this operator, we obtain a more compact and efficient feature representation for each vertex, which is important for training our segmentation model. \autoref{fig:framework}-B shows the node feature generation process.

\paragraph{Graph Convolution Module} We propose our graph convolution module $F_g(.)$, based on node classification with graph convolution operator \cite{kipf2016semi}, at the top of our grid-based visual graph of the nodes to learn feature representations encoding the relationship and neighborhood between the nodes. First, initial node features $f_c$ are reformatted into node feature matrix $D_{f_c} \in \mathbb{R}^{N \,\times\,64}$ for graph-based processing. Then, $D_{f_c}$ and $A$ are fed into our graph convolution module to generate graph features combined with initial node features by a skip connection, which results in final node feature matrix $D_{f_{g+c}} \in \mathbb{R}^{N \,\times\,96}$. Class prediction for each node, to decide whether the patch of the node contains a vessel branch or not, is made by the last graph convolution layer by using those final node features. There are, in total, eleven graph convolution layers in the network, in which the input to layer $i$ is concatenated with the output of layer $i+2$ by local skip connections to be passed into the layer $i+3$ as shown in \autoref{fig:framework}-C. These skip connections enable the network to have easier gradient flow inside $F_g(.)$ and also between $F_g(.)$ and $F_c(.)$.

\paragraph{Inference} Our inference module (shown in \autoref{fig:framework}-D) is responsible for providing a smooth transition between node predictions and their pixel-wise correspondences. After the graph convolution module classifies each node as foreground or background, the class predictions are extended to $n \times n$ spatial areas that correspond to the nodes in the input image, resulting in a segmentation map in the spatial domain. Our approach differs depending on the size of the node patches. If we use $1 \times 1$ patches, each pixel is treated as a node, and the node predictions are directly accepted as pixel predictions for the segmentation map. However, if we use larger patch sizes such as $2 \times 2$, each node represents a region of pixels. In this case, we use nearest neighbor interpolation to map the class of each node to its corresponding $2 \times 2$ region. This allows us to produce a pixel-wise segmentation map even when the node patches are larger than a single pixel. This way, our mapping function serves as a transition from the graph domain to the spatial domain, which facilitates the interpretation of visual graphs in the image space.

%\Rui{Is the mapping function our novelty here? If yes, we should emphasize here}


\subsection{Losses} clDice \cite{shit2021cldice} has proven to be an effective loss for preserving continuity; therefore, we employ it for training our graph-based approach. The general idea lying behind clDice loss is to measure the centerline connectivity on the spatial domain from the intersection of segmented and ground-truth vessels with their skeletons. This makes graph-based approaches inconvenient to be trained with clDice. To alleviate this problem, we introduce a reshaping function that puts node predictions of regular visual graphs into a 2D image form to imitate the shape and structure of vessels.

%Our framework is trained using clDice loss \cite{shit2021cldice}, which was proposed as a centerline continuity metric. clDice loss is utilized to generate accurate topological segmentation of tubular structures by preserving their centerline continuity. 



==> SCOPE_ arXiv/chapters/4_results.tex <==
\section{Experiments and Results}
This section provides a comprehensive evaluation of the proposed method for segmenting retinal vessels based on various metrics. The evaluation is carried out on the CHASE\textunderscore DB1 \cite{fraz2012ensemble} and FIVES~\cite{jin2022fives} datasets. We compare our methodology with existing studies, perform an ablation study of graph construction components, and use baseline models such as DRIU \cite{maninis2016deep} and a more recent adaption of UNet (\uinet{}) \cite{kerfoot2019left}. We also evaluate the continuity of vessel segmentations using pre-trained weights from previous studies, including SGL \cite{zhou2021study} and FR-UNet \cite{liu2022full} for the CHASE dataset \cite{fraz2012ensemble}.

\begin{table}[htbp]
    \centering
    \caption{Qualitative results on FIVES \cite{jin2022fives} dataset}
    \label{figs:qualitative} \vspace{-10pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c@{\hskip 0.10cm} c@{\hskip 0.10cm} c@{\hskip 0.10cm} c@{\hskip 0.10cm} c@{\hskip 0.10cm}}
        \hline
        Segmentation Map & GT & \methodName{} (Ours) & DRIU \cite{maninis2016deep} & \uinet{} \cite{ronneberger2015u} \\
        \hline
        \multirow[b]{2}{*}[5.2em]{
        \includegraphics[width=4.3cm,height=4.3cm]{figures/samples_2/main.pdf}}
        & \includegraphics[width=2.1cm]{figures/samples_2/zoom_1_gt.pdf} & \includegraphics[width=2.1cm]{figures/samples_2/zoom_1_scope.pdf} & \includegraphics[width=2.1cm]{figures/samples_2/zoom_1_driu.pdf} & \includegraphics[width=2.1cm]{figures/samples_2/zoom_1_unet.pdf} \\
        & \includegraphics[width=2.1cm]{figures/samples_2/zoom_2_gt.pdf} & \includegraphics[width=2.1cm]{figures/samples_2/zoom_2_scope.pdf} & \includegraphics[width=2.1cm]{figures/samples_2/zoom_2_driu.pdf} & \includegraphics[width=2.1cm]{figures/samples_2/zoom_2_unet.pdf}
    \end{tabular}
    }
\end{table}


\begin{table}[tbh]
\caption{Comparison to SOTA on CHASE \textunderscore DB1~\cite{fraz2012ensemble}.}
\label{tab:chase_comparison} \vspace{-10pt}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c c c |c c c c|}
\hline
 &  \multicolumn{3}{c|}{\segmentation{}} & \multicolumn{4}{c|}{\continuity{}} \\ \hline
Method     & Pre (\%) $\uparrow$& Rec (\%) $\uparrow$ &Dice(\%)$\uparrow$& clDice (\%) $\uparrow$ & $error_{\beta_{0}}$ $\downarrow$ & $error_{\beta_{1}}$ $\downarrow$ & $error_{\chi}$ $\downarrow$\\ \hline
\uinet{} \cite{kerfoot2019left}         &     0.78     &  0.80    & 0.79   &    0.74         &            59.8 & 2.8     &    61.2           \\ 
DRIU \cite{maninis2016deep}          & 0.79         &0.80    &  0.79    &0.74           &37.8& 4.2                 &35.1               \\ 
FR-UNet \cite{liu2022full} & 0.76 & \textbf{0.88} & 0.80 & 0.73 & 61.0 & 2.8 & 64.4 \\ 
SGL \cite{zhou2021study} & \textbf{0.79} & 0.87 & \textbf{0.82} & 0.75 & 42.6 & 2.3 & 46.0 \\ 
\methodName{} (Ours) &    0.75      &      0.86  & 0.80 &      \textbf{0.81}       &    \textbf{24.2}& \textbf{1.6}             &     \textbf{22.7}          \\ \hline
\end{tabular}
}
\end{table}



\subsection{Datasets}
\textbf{CHASE\textunderscore DB1}\cite{fraz2012ensemble} has 28 fundus images of size 999 x 960. We split the dataset into two subsets, with the first 20 used for training and the last 8 for testing.

\noindent\textbf{FIVES} \cite{jin2022fives} is composed of 800 fundus images with 2048$\times$2048 resolution split into four equally-distributed subcategories of different diseases: Age-related Macular Degeneration (AMD), Diabetic Retinopathy (DR), Glaucoma, and Normal (see \autoref{figs:sampleFives}). Train and test sets consist of 600 and 200 images, respectively. %We adhere to this configuration for the evaluation of our method on this dataset.

%\textbf{CHASE\textunderscore DB1} consists of 28 coloured retinal images and serves as a powerful benchmark in retinal vessel segmentation task. Therefore, we use CHASE\textunderscore DB1 mainly for the comparison between our methods and other SOTA methods in terms of both segmentation and topological metrics. To enforce fair comparison, we follow the same setting as (Names of other papers), which is first 20 images for training and last 8 images for testing.

%\\\indent \textbf{Fives} The FIVES dataset consists of 800 high-resolution color fundus photographs with pixelwise manual annotation. It divided equally into 4 categories in terms of diseases: age-related mascular degeneration(AMD), diabetic retinopathy(DR), glaucoma and normal class. We choose 


\subsection{Experimental Setup}
All values reported for the \uinet{} \cite{kerfoot2019left} and DRIU~\cite{maninis2016deep} experiments are based on our own implementation. We train the baseline models as well as ours on the FIVES~\cite{jin2022fives} dataset for 100 epochs, using Adam optimizer with a batch size of 8 and weight decay of $1e^{-3}$. We set the learning rate to $1e^{-2}$ for \uinet{} \cite{alom2019recurrent} and $1e^{-3}$ for DRIU~\cite{maninis2016deep}. To address the domain shift problem and adapt the pre-trained weights to the context of CHASE~\cite{fraz2012ensemble}, we fine-tuned the baseline models that are pre-trained on FIVES \cite{jin2022fives}. We used the same hyperparameters for both datasets unless specified. The models were trained on CHASE for 200 epochs. To be consistent with the original paper, we used cross-entropy loss for both datasets during training. We downsample the images to $512 \times 512$ resolution for training and testing in both datasets.
% \iffalse
% Our experimental setup comprises two stages for baseline models and our proposed method, respectively.  First, \uinet{} and DRIU architectures, as baseline, are trained on FIVES dataset 100 epochs with batch size of 8 and weight decay of 1e -3 by using Adam optimizer. Their training scheme only differentiates in terms of learning rate due to their complexity. While \uinet{} is trained with $1e-2$ learning rate, using a smaller one for DRIU due to its more complex structure, which is equal to 1e -3, is considered to be a better option. Then, we train these two base architectures with CHASE, yet we follow slightly different approach. Since FIVES is a large dataset diversified with 4 retinal diseases, it is easier to learn the topological structure of vessels, but this is not the case for CHASE\textunderscore DB1 due to its limited number of training set. That is the main reason why we prefer to take the baselines pre-trained on FIVES and fine-tune on CHASE instead of directly training with it. We completely use same hyper-parameters as in FIVES, but to alleviate the domain shift problem and thereby making pretrained weights adapted to the context in CHASE\textunderscore DB1, we prefer to train 200 epochs. To stay in the same line with the original setting in the papers, these models are trained with cross entropy loss for both datasets.
% \fi

%We also trained our proposed method on both FIVES \cite{jin2022fives}, and CHASE\textunderscore DB1 \cite{fraz2012ensemble} datasets. 
For our proposed method, the node feature generator is trained individually on each dataset using the same hyper-parameters as the DRIU \cite{maninis2016deep} baseline. We incorporate the node feature generator into our graph convolution module, and it is jointly trained with graph-integrated clDice loss \cite{shit2021cldice}. We set the learning rate for training \methodName{} on FIVES to $4e^{-4}$, and the weight decay to $5e^{-3}$. For CHASE \cite{fraz2012ensemble}, we adhere to the same configuration as in FIVES \cite{jin2022fives} except for the number of training epochs which is 200 due to the limited size of the dataset. 
%The graph-integrated clDice loss receives the graph node predictions as spatial input in a reshaped form and backpropagates the gradients through the nodes
% \iffalse
% As a second stage of experimental setup, our proposed method is trained with both datasets, for each of which it goes through sequential 2-step training process. At first, node feature generator of \methodName{}  is individually trained on FIVES and CHASE\textunderscore DB1 datasets with completely same configuration and same hyper-parameters as DRIU baseline, but using clDice loss. Then, it is plugged in our graph convolution module and they are jointly trained with graph-integrated clDice loss, which receives graph node predictions as spatial input in reshaped form and back-propagates the gradients through the nodes. \methodName{}  is joint-trained on FIVES 100 epochs with batch size of 2, learning rate of 4e -4, and weight decay of 5e -3 by using Adam optimizer. For CHASE\textunderscore DB1 dataset, we also adhere to same training configuration as in FIVES except 200 epochs due to the limited size of the dataset. 
% \fi
\paragraph{Evaluation Metrics}
Given that the intended goal in this paper is to evaluate the continuity and topology of vessels rather than pure pixel-wise metrics, we use four main topological metrics in our results: (i) clDice \cite{shit2021cldice} evaluating the topological continuity of tubular structures, (ii) $\beta_0$ (Betti zero) \cite{clough2020topologicalBetti} that counts the number of connected components in a topological space,  (iii) $\beta_1$ (Betti one) \cite{clough2020topologicalBetti} indicating the number of independent loops or cycles in the space, and   (iv) $\chi$ (Euler) characteristic \cite{beltramo2021euler} that is a topological invariant quantifying the connectivity and complexity anatomical structure by counting the number of its connected components, holes, and voids, we utilize them as $error_{\beta_{0}}$, $error_{\beta_{1}}$, and $error_{\chi}$ to compare ground truth with predicted results. %It should be noted that these metrics represent different aspects of continuity, with clDice focusing on center-line connectivity, and Bettis considering the number of disconnected components. By evaluating these metrics together, we can get a comprehensive evaluation of connectivity.
%\Rui{These continuity metrics have a different focus: clDice focuses on center-line connectivity while Bettis focuses on the number of disconnected components. By evaluating these metrics together, we can get a comprehensive evaluation of connectivity.}
%\Amr{We don't need to mention voids here because we're dealing with 2d images not 3d. Maybe also mention that we're taking the absolute difference since other papers are dividing and so we don't see how \textbf{many} additional holes or connected components there are on average in the image. their error calculation somehow obfuscates how off their topology is. Also reference is good!}



\subsection{Results}
Comparison of vessel segmentation models on CHASE dataset \cite{fraz2012ensemble} using pixel-wise and connectivity metrics shown on \autoref{tab:chase_comparison}, indicates that our model significantly outperforms other methods in continuity metrics and comparable pixel-wise metrics values, outperforming state-of-the-art architectures and two baseline models, a recent modification of \uinet{} \cite{alom2019recurrent}, and DRIU~\cite{maninis2016deep}.

% \iffalse
% Table1: We compared our model with the state-of-the-art architectures in vessel segmentation task on CHASE\_DB1 dataset, we utilized their pre-trained models and inference with both segmentation and topological metrics. Besides that, we also included UNet \cite{kerfoot2019left} and DRIU \cite{maninis2016deep} as our two baseline models. \\
% Table 1 shows that our model achieves the best continuity results among all models. This demonstrates the superiority of SCOPE: The patch-wise sampled nodes go through a message-passing step during graph convolutions. The vessel nodes are more likely to connect and the non-vessel nodes are eliminated. In the end, the nodes will try to imitate the vessels and therefore focus more on the continuity of vessel structures. Besides, our model has also achieved a comparable pixel-wise segmentation result. This shows that we're not sacrificing pixel-wise predictions for continuity preservation. 
% \fi


\begin{table}[tb]
\centering
\caption{\textbf{Comparison with previous work.} We present the results of our methodology compared to previous work on the FIVES \cite{jin2022fives} dataset.}
\label{tabs:fives} %\vspace{-10pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|c c c|c c c c|}
\hline
& & \multicolumn{3}{c|}{\segmentation{}} & \multicolumn{4}{c|}{\continuity{}} \\ \hline
Class           & Architecture &Pre (\%) $\uparrow$& Rec (\%) $\uparrow$ & Dice(\%) $\uparrow$ & clDice (\%) $\uparrow$ & $error_{\beta_{0}}$ $\downarrow$ & $error_{\beta_{1}}$ $\downarrow$ & $error_{\chi}$ $\downarrow$\\ \hline
\multirow{3}{*}{AMD} &\uinet{} \cite{kerfoot2019left}&    0.88        &           0.93&  0.90  &    0.87&        72.8&    4.3&    71.1   \\  
                   &DRIU \cite{maninis2016deep}&              0.87&           \textbf{0.95}&  \textbf{0.91} &  0.87   &        57.8&    2.7&    57.1   \\ 
                   & \methodName{} (Ours)&              \textbf{0.90}&           0.92&  \textbf{0.91}   &   \textbf{ 0.94}&        \textbf{6.7}&   \textbf{2.6}&   \textbf{ 7.9}   \\ \hline
\multirow{3}{*}{DR} &\uinet{} \cite{kerfoot2019left}&              0.85&           0.92& 0.89  &     0.84&        89.5&    4.1&    83.8   \\ 
                   &DRIU \cite{maninis2016deep}&              0.85&           \textbf{0.94}&  0.89  &    0.85&      64.3&    3.8 &60.5  \\  
                   &\methodName{} (Ours)&              \textbf{0.91}&           0.89&  \textbf{0.90}   &   \textbf{0.92}&        \textbf{10.6}&    \textbf{3.0}&    \textbf{14.0 }  \\ \hline
\multirow{3}{*}{Glaucoma} &\uinet{} \cite{kerfoot2019left}             &           0.84&        0.90&   0.87   &  0.83&    87.6&    5.6&83.2   \\ 
                   &DRIU \cite{maninis2016deep}             &           0.87&        \textbf{0.92}&  \textbf{0.89}   &     \textbf{ 0.85}&    51.2&    \textbf{3.4}&   53.1\\ 
                  &\methodName{} (Ours)              &          \textbf{0.91}&        0.77&   0.81   &   0.83&    \textbf{5.4}&  4.5&   \textbf{11.9}\\ \hline
\multirow{3}{*}{Normal} &\uinet{} \cite{kerfoot2019left}            &         0.87&        0.90&    \textbf{0.88}  &    0.84&    141.6&    8.8&123.3   \\ 
                   &DRIU \cite{maninis2016deep}             &          0.83&       \textbf{ 0.94}&    \textbf{0.88}   &   0.84&    138.9&    6.4&   124.8\\ 
                   &\methodName{} (Ours)              &         \textbf{0.89}&        0.87&  \textbf{0.88}   &   \textbf{0.89}&    \textbf{14.0}&    \textbf{4.2}&   \textbf{13.2}\\
                   \hline
\multirow{3}{*}{Average} &\uinet{} \cite{kerfoot2019left}             &         0.85&        0.90&    0.87  &    0.83&    98.0&    5.6&90.5   \\  
                   &DRIU \cite{maninis2016deep}              &          0.85&       \textbf{ 0.92}&    \textbf{0.88}   &   0.84&    73.8&    4.5&   70.4\\ 
                   &\methodName{} (Ours)              &         \textbf{0.90}&        0.85&  0.85   &   \textbf{0.87}&    \textbf{12.1}&    \textbf{3.7}&   \textbf{14.4}\\ \hline
\end{tabular}
}
\end{table}


We also validate our proposed method on the newly released FIVES dataset \cite{jin2022fives} in \autoref{tabs:fives}. To the best of our knowledge, no method has reported results on the FIVES \cite{jin2022fives} dataset. To this end, we compare our model against two competitive models based on the results obtained on CHASE~\cite{fraz2012ensemble}, namely \uinet{} \cite{kerfoot2019left}, and DRIU \cite{maninis2016deep}, as the baselines on FIVES \cite{jin2022fives}. %\yousef{can we argue something else to say why we choose these two?}\ehsan{writing a sentence reason why you selected these is good! } 
The results in \autoref{tabs:fives} show that our model significantly outperforms the two baselines in connectivity metrics $error_{\beta_0}$, $error_{\beta_1}$, $error_{\chi}$, and clDice, while achieving better or comparable results in pixel-wise metrics. This improvement in connectivity metrics indicates that our model enforces the preservation of topological information, while other methods do not strictly enforce it. Our qualitative results in \autoref{figs:qualitative} also support that where other baselines introduced discontinuity to the topology, our method preserves it. Note that since pixel-wise metrics are only sensitive to the pixels, they cannot represent connectivity.
%\Amr{technicality but our connectivity metrics are $error_{\beta_0}$, $error_{\beta_1}$, $error_{\chi}$ counting the connected components of the inference on their own doesn't tell us anything}

% However, this also leads to the relatively worse recall, since our model always tries to eliminate tiny disconnected vessel segments, it tends to classify pixels as 'background', which in fact should be a vessel. This will increase the FN and lead to worse recall. Actually this reflects why we should attach more importance on continuity metrics, because pixel-wise segmentation metrics focus too much on the correctness of pixel prediction but overlook the relation ship between neighbouring pixels. \\
% Different diseases are having different effects on the retinal vessels, this means that, even the ground-truth has discontinuity.






% \begin{table}[htb]
% \centering
% \caption{\textbf{Comparison to previous work.} We present the results of our methodology compared to previous work on the FIVES \cite{jin2022fives} dataset.}
% \label{tabs:fives}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% & & \multicolumn{3}{c|}{\segmentation{}} & \multicolumn{4}{c|}{\continuity{}} \\ \hline
% Class           & Architecture &Pre (\%) $\uparrow$& Rec (\%) $\uparrow$ & Dice(\%) $\uparrow$ & clDice (\%) $\uparrow$ & $error_{\beta_{0}}$ $\downarrow$ & $error_{\beta_{1}}$ $\downarrow$ & $error_{\chi}$ $\downarrow$\\ \hline
% \multirow{3}{*}{AMD} &\uinet{} \cite{kerfoot2019left}&    0.88        &           0.93&  0.90  &    0.87&        72.8&    4.3&    71.1   \\ \cline{2-9} 
%                    &DRIU \cite{maninis2016deep}&              0.87&           \textbf{0.95}&  \textbf{0.91} &  0.87   &        57.8&    2.7&    57.1   \\ \cline{2-9} 
%                    & \methodName{} (Ours)&              \textbf{0.90}&           0.92&  \textbf{0.91}   &   \textbf{ 0.94}&        \textbf{6.7}&   \textbf{2.6}&   \textbf{ 7.9}   \\ \hline\hline
% \multirow{3}{*}{DR} &\uinet{} \cite{kerfoot2019left}&              0.85&           0.92& 0.89  &     0.84&        89.5&    4.1&    83.8   \\ \cline{2-9} 
%                    &DRIU \cite{maninis2016deep}&              0.85&           \textbf{0.94}&  0.89  &    0.85&      64.3&    3.8 &60.5  \\ \cline{2-9} 
%                    &\methodName{} (Ours)&              \textbf{0.91}&           0.89&  \textbf{0.90}   &   \textbf{0.92}&        \textbf{10.6}&    \textbf{3.0}&    \textbf{14.0 }  \\ \hline\hline
% \multirow{3}{*}{Glaucoma} &\uinet{} \cite{kerfoot2019left}             &           0.84&        0.90&   0.87   &  0.83&    87.6&    5.6&83.2   \\ \cline{2-9} 
%                    &DRIU \cite{maninis2016deep}             &           0.87&        \textbf{0.92}&  \textbf{0.89}   &     \textbf{ 0.85}&    51.2&    \textbf{3.4}&   53.1\\ \cline{2-9} 
%                   &\methodName{} (Ours)              &          \textbf{0.91}&        0.77&   0.81   &   0.83&    \textbf{5.4}&  4.5&   \textbf{11.9}\\ \hline\hline
% \multirow{3}{*}{Normal} &\uinet{} \cite{kerfoot2019left}            &         0.87&        0.90&    \textbf{0.88}  &    0.84&    141.6&    8.8&123.3   \\ \cline{2-9} 
%                    &DRIU \cite{maninis2016deep}             &          0.83&       \textbf{ 0.94}&    \textbf{0.88}   &   0.84&    138.9&    6.4&   124.8\\ \cline{2-9} 
%                    &\methodName{} (Ours)              &         \textbf{0.89}&        0.87&  \textbf{0.88}   &   \textbf{0.89}&    \textbf{14.0}&    \textbf{4.2}&   \textbf{13.2}\\
%                    \hline\hline
% \multirow{3}{*}{Average} &\uinet{} \cite{kerfoot2019left}             &         0.85&        0.90&    0.87  &    0.83&    98.0&    5.6&90.5   \\ \cline{2-9} 
%                    &DRIU \cite{maninis2016deep}              &          0.85&       \textbf{ 0.92}&    \textbf{0.88}   &   0.84&    73.8&    4.5&   70.4\\ \cline{2-9} 
%                    &\methodName{} (Ours)              &         \textbf{0.90}&        0.85&  0.85   &   \textbf{0.87}&    \textbf{12.1}&    \textbf{3.7}&   \textbf{14.4}\\ \hline
% \end{tabular}
% }
% \end{table}

% \ehsan{give your method a name and use that in the tables; also add the citation of the previous works in the tables} 

% \ehsan{any qualitative results?}

\begin{table}[t]
    \centering
    \caption{Sample Images and Ground-Truth in Fives Dataset}
    \label{figs:sampleFives}\vspace{-10pt}
    \begin{tabular}{c c c c c c}
        \hline
        & AMD & DR & Glaucoma & Normal \\
        %\hline
        \rotatebox{90}{Image} & \includegraphics[width=2cm]{figures/fives/image/img_A.pdf} & \includegraphics[width=2cm]{figures/fives/image/img_D.pdf} &
        \includegraphics[width=2cm]{figures/fives/image/img_G.pdf} &
        \includegraphics[width=2cm]{figures/fives/image/img_N.pdf} \\
        %\hline
        \rotatebox{90}{GT} & \includegraphics[width=2cm]{figures/fives/label/label_A.pdf} & \includegraphics[width=2cm]{figures/fives/label/label_D.pdf} &
        \includegraphics[width=2cm]{figures/fives/label/label_G.pdf} &
        \includegraphics[width=2cm]{figures/fives/label/label_N.pdf} \\
        %\hline
        \rotatebox{90}{Pred} & \includegraphics[width=2cm]{figures/fives/prediction/pred_A.pdf} & \includegraphics[width=2cm]{figures/fives/prediction/pred_D.pdf} &
        \includegraphics[width=2cm]{figures/fives/prediction/pred_G.pdf} &
        \includegraphics[width=2cm]{figures/fives/prediction/pred_N.pdf} \\
        %\hline
    \end{tabular}
\end{table}

In our ablation studies \autoref{tabs:ablation}, we analyze the effect of the objective function and patch size on the inferences. We first note the strong effect of clDice \cite{shit2021cldice} in both pixel-wise Metrics and connectivity metrics. Given that clDice \cite{shit2021cldice} is specifically designed for tubular structure, it can be inferred that increasing the patch size causes over-segmentation and damages the center-line connectivity and therefore the segmentation results. This can be observed in \autoref{tabs:ablation}, where the 2$\times$2 patching actually worsens the results. %We hypothesize that this is due to the glaucoma dataset specifically where bigger patch sizes allow for more convolutions with empty areas of the image, which brings the overall performance down. 
%Our hypothesis that bigger patching sizes create better topological results remains to be seen. 

%We also note that pixel-wise metrics are not enforcing the preservation of connectivity. 
%\Amr{Maybe if we can just point out that it's obvious that increasing the patch sizes decreases the pixel wise metrics. But we hypothesize that it's good for connectivity.} \Rui{We don't need to say 'surprisingly ' here, we just say that increasing patch sizes are causing over-segmentation and damaging center-line connectivity and segmentation results.}

\begin{table}[t]
\caption{Ablation study on different loss functions and patch sizes on FIVES \cite{jin2022fives}.} 
\label{tabs:ablation}\vspace{-10pt}
% The results are obtained on the Fives \cite{jin2022fives} dataset
\resizebox{\textwidth}{!}{
\centering
\begin{tabular}{|l|c|ccc|cccc|}
\hline
 & & \multicolumn{3}{c|}{\segmentation{}} & \multicolumn{4}{c|}{\continuity{}} \\  \cline{3-9}
\multirow{4}{*}{\rotatebox{90}{Loss}}  & & Pre (\%) $\uparrow$ & Rec (\%) $\uparrow$ & Dice(\%) $\uparrow$ & clDice (\%) $\uparrow$ & $error_{\beta_{0}}$ $\downarrow$ & $error_{\beta_{1}}$ $\downarrow$ & $error_{\chi}$ $\downarrow$\\  \cline{3-9}

 & CE Loss            &        0.89        &  0.77  &  0.81       &      0.78       &       52.6 & 4.4            &      53.6  \\    %\cline{2-9}
& CE + clDice & \textbf{0.90}  & 0.81 & \textbf{0.85} & 0.84  &    22.7 & 4.2                &     27.1  \\ %\cline{2-9}
 & clDice & \textbf{0.90} & \textbf{0.85} & \textbf{0.85} & \textbf{0.87} & \textbf{12.1} & \textbf{3.7} & \textbf{14.4} \\ %
 \hline \hline
  %\hline
% \multirow{3}{*}{n} & &  Pre ($\%$) $\uparrow$ & Rec ($\%$) $\uparrow$ &Dice(\%)$\uparrow$& clDice ($\%$) $\uparrow$ &$error_{\beta_{0}}$ $\downarrow$ & $error_{\beta_{1}}$ $\downarrow$ & $error_{\chi}$ $\downarrow$\\  \cline{3-9}
 \multirow{2}{*}{n} & 1$\times$1      &      \textbf{0.90}          &       \textbf{0.85}  & \textbf{0.85}  &     \textbf{0.87}         &        \textbf{ 12.1}          & \textbf{ 3.7 }   & \textbf{14.4 }\\  %\cline{2-9}
& 2$\times$2      &       0.71         &  0.84        & 0.76  &  0.83            &       12.83            &  5.13    & 17.37\\  \hline
\end{tabular}
}
\end{table}

%%\yousef{Need opinion regarding these qualitative and ablation studies } \ehsan{reading through results}




%%%%%%%%%%% Move to discussions %%%%%%%%%%%%%
% When we compare this idea with their counterparts, we see that using super-pixels \cite{wu2022graph} and vessel bifurcations \cite{yu2022vessel} to instantiate the graph nodes are also possible. However, these approaches actually tend to make graph construction process more costly and complicated. First of all, they require some preprocessing operations like SLIC \cite{achanta2012slic} and corner-detection \cite{shi1994good} for the extraction of super-pixel clusters and detection of bifurcations. Secondly, since their node representations are not in a regular form, some clusters assigned to the nodes need to be defined and the features of pixels inside these clusters requires to be averaged for vertex feature initialization process. These reasons actually led us to make use of more concise and regular graph construction approach. Besides, we adopted the strategy of sampling the vertices on everywhere inside the image instead of only at the top of vessel regions in order to investigate the vessels and their mutual spatial relationship. 

% In this scenario, each patch can cover a background region, a particular segment of foreground vessels or a bit of both. Even if covering some vessels seems to be sufficient for the vertex of the corresponding patch to be classified as foreground, the size of those patches, in fact, tend to affect the result of node classification as well as the continuity of segmented vessels. In other words,  including some vessels does not guarantee that the node of relevant patch will be absolutely classified under foreground category because the dominance of background region in the patch can be misleading, that is the case quite observable in large patches. On the other hand, choosing a smaller value for  would definitely make the patches more isolated. Hence, each patch will be mostly or even completely dedicated to background or foreground. In addition to this, the patches in smaller size will hit a small part of solely one vessel branch; thus, side-by-side connected nodes will be a representative of one full vessel branch, which makes the continuity more understandable for the network. With these motivations, we specifically opted for the size of $1 \times 1$ and $2 \times 2$ patching. 

==> SCOPE_ arXiv/chapters/5_conclusion.tex <==
\section{Conclusion}
In conclusion, preserving shape continuity is critical in medical imaging as it can impact the accuracy of medical diagnoses. Unfortunately, traditional deep learning methods often neglect this aspect, leading to inaccurate predictions. In this work, we proposed a graph-based approach that enforces shape continuity in medical segmentation by encoding it as a graph constraint. Our method significantly improved shape continuity metrics compared to traditional methods while maintaining or improving segmentation performance. By enforcing shape continuity, our approach can potentially improve the accuracy of medical diagnoses, especially in structures such as vessels, where continuity is critical.
